Gini representations of skewness, kurtosis and higher-order moments

We provide pairwise-difference (Gini-type) representations of higher-order central moments for both general random variables and empirical moments. Such representations do not require a measure of location. For third and fourth moments, this yields pairwise-difference representations of skewness and kurtosis coefficients. We show that all central moments possess such representations, so no reference to the mean is needed for moments of any order. This is done by considering i.i.d. replications of the random variables considered, by observing that central moments can be interpreted as covariances between a random variable and powers of the same variable, and by giving recursions which link the pairwise-difference representation of any moment to lower order ones.

==> DufourC1F.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DufourC1F.tex 
%% Latex file 
%% Version: 1 March 2002; 5 February 2011; 14 July 2011; 15 July 2011; 18 July 2011; 
%%          19 July 2011; 23 July 2016; 25 January 2017
%% Commands for text in French
%% French translations of names in DufourC1.tex

%\usepackage[francais]{babel}
%\usepackage[french]{babel}
\usepackage[frenchb]{babel}  %% Frontpage footnote not well formatted
%\usepackage{frenchle}  %% For paper in French. Frequent compilation errors.

\providecommand{\theoremname}{\spth Th\'eor\`eme}
\providecommand{\acknowledgementname}{\spth Reconnaissance}
\providecommand{\algorithmname}{\spth Algorithme}
\providecommand{\assumptionname}{\spth Hypoth\`ese}
\providecommand{\axiomname}{\spth Axiome}
\providecommand{\casename}{\spth Cas}
\providecommand{\claimname}{\spth Affirmation}
\providecommand{\conclusionname}{\spth Conclusion}
\providecommand{\conditionname}{\spth Condition}
\providecommand{\conjecturename}{\spth Conjecture}
\providecommand{\corollaryname}{\spth Corollaire}
\providecommand{\criterionname}{\spth Crit\`ere}
\providecommand{\definitionname}{\spth D\'efinition}
\providecommand{\examplename}{\spth Exemple}
\providecommand{\exercisename}{\spth Exercice}
\providecommand{\lemmaname}{\spth Lemme}
\providecommand{\notationname}{\spth Notation}
\providecommand{\problemname}{\spth Probl\`eme}
\providecommand{\proofname}{\sppr D\'emonstration}
\providecommand{\proofthname}{\sppr D\'emonstration}
\providecommand{\propositionname}{\spth Proposition}
\providecommand{\reflistname}{\spth R\'ef\'erences}
\providecommand{\remarkname}{\spth Remarque}
\providecommand{\solutionname}{\spth Solution}
\providecommand{\statementname}{\spth Affirmation}
\providecommand{\summaryname}{\spth R\'esum\'e}

\renewcommand{\theoremname}{\spth Th\'eor\`eme}
\renewcommand{\acknowledgementname}{\spth Reconnaissance}
\renewcommand{\algorithmname}{\spth Algorithme}
\renewcommand{\assumptionname}{\spth Hypoth\`ese}
\renewcommand{\axiomname}{\spth Axiome}
\renewcommand{\casename}{\spth Cas}
\renewcommand{\claimname}{\spth Affirmation}
\renewcommand{\conclusionname}{\spth Conclusion}
\renewcommand{\conditionname}{\spth Condition}
\renewcommand{\conjecturename}{\spth Conjecture}
\renewcommand{\corollaryname}{\spth Corollaire}
\renewcommand{\criterionname}{\spth Crit\`ere}
\renewcommand{\definitionname}{\spth D\'efinition}
\renewcommand{\examplename}{\spth Exemple}
\renewcommand{\exercisename}{\spth Exercice}
\renewcommand{\lemmaname}{\spth Lemme}
\renewcommand{\notationname}{\spth Notation}
\renewcommand{\problemname}{P\spth robl\`eme}
\renewcommand{\proofname}{\sppr D\'emonstration}
\renewcommand{\proofthname}{\sppr D\'emonstration}
\renewcommand{\propositionname}{\spth Proposition}
\renewcommand{\reflistname}{\spth R\'ef\'erences}
\renewcommand{\remarkname}{\spth Remarque}
\renewcommand{\solutionname}{\spth Solution}
\renewcommand{\statementname}{\spth Affirmation}
\renewcommand{\summaryname}{\spth R\'esum\'e}

\providecommand{\listttheoremnameb}{\sectitlesize Liste de d\'efinitions, propositions et th\'eor\`emes}
\renewcommand{\listttheoremnameb}{\sectitlesize Liste de d\'efinitions, hypoth\`eses, propositions et th\'eor\`emes}


\providecommand{\proofof}{Preuve de }
\renewcommand{\proofof}{Preuve de }

\providecommand{\capcorollary}[1]{\captiontheorem{Corollaire}{#1}}
\providecommand{\capdefinition}[1]{\captiontheorem{D\'efinition}{#1}}
\providecommand{\capexample}[1]{\captiontheorem{Exemple}{#1}}
\providecommand{\caplemma}[1]{\captiontheorem{Lemme}{#1}}
\providecommand{\capproposition}[1]{\captiontheorem{Proposition}{#1}}
\providecommand{\capremark}[1]{\captiontheorem{Remarque}{#1}}
\providecommand{\capstatement}[1]{\captiontheorem{}{#1}}
\providecommand{\captheorem}[1]{\captiontheorem{Th\'eor\`eme}{#1}}


\renewcommand{\capcorollary}[1]{\captiontheorem{Corollaire}{#1}}
\renewcommand{\capdefinition}[1]{\captiontheorem{D\'efinition}{#1}}
\renewcommand{\capexample}[1]{\captiontheorem{Exemple}{#1}}
\renewcommand{\caplemma}[1]{\captiontheorem{Lemme}{#1}}
\renewcommand{\capproposition}[1]{\captiontheorem{Proposition}{#1}}
\renewcommand{\capremark}[1]{\captiontheorem{Remarque}{#1}}
\renewcommand{\capstatement}[1]{\captiontheorem{}{#1}}
\renewcommand{\captheorem}[1]{\captiontheorem{Th\'eor\`eme}{#1}}


\providecommand{\harvardand}{et}
\renewcommand{\harvardand}{et}

\providecommand{\standardthanks}{}
\renewcommand{\standardthanks}{Cette recherche a b\'{e}n\'{e}fici\'{e}
  du support financier de la Chaire William Dow (McGill University), 
  de la Banque du Canada (Bourse de recherche), 
  d'une Bourse Guggenheim, de la Bourse Konrad-Adenauer
  (Fondation Alexander von Humboldt, Allemagne),
  du Conseil de recherche en sciences humaines du Canada, du
  Conseil de recherche en sciences naturelles et en g\'{e}nie du
  Canada, du R\'{e}seau canadien de centres d'excellence (projet MITACS), et du
  Fonds de recherche sur la soci\'{e}t\'{e} et la culture
  (Qu\'{e}bec).}

\providecommand{\standardthanksOld}{}
\renewcommand{\standardthanksOld}{Cette recherche a b\'{e}n\'{e}fici\'{e}
  du support financier de la Chaire de recherche du Canada en
  \'{e}conom\'{e}trie, d'une Bourse Guggenheim, de la Bourse Konrad-Adenauer
  (Fondation Alexander von Humboldt, Allemagne),
  du Conseil de recherche en sciences humaines du Canada, du
  Conseil de recherche en sciences naturelles et en g\'{e}nie du
  Canada, de la Fondation Alexander von Humboldt (Allemagne), du
  R\'{e}seau canadien de centres d'excellence (projet MITACS), du
  Fonds de recherche sur la soci\'{e}t\'{e} et la culture
  (Qu\'{e}bec), et du Fonds de recherche sur la nature et les
  technologies (Qu\'{e}bec), et d'une Bourse
  Killam (Conseil des Arts du Canada).}

\providecommand{\standardthanksIFM}{}
\renewcommand{\standardthanksIFM}{Cette recherche a b\'{e}n\'{e}fici\'{e}
  du support financier de la Chaire William Dow (McGill University), 
  de la Banque du Canada (Bourse de recherche),
  d'une Bourse Guggenheim, de la Bourse Konrad-Adenauer
  (Fondation Alexander von Humboldt, Allemagne),
  du Conseil de recherche en sciences humaines du Canada, du
  Conseil de recherche en sciences naturelles et en g\'{e}nie du
  Canada, du R\'{e}seau canadien de centres d'excellence (projet MITACS), et du
  Fonds de recherche sur la soci\'{e}t\'{e} et la culture
  (Qu\'{e}bec).}
  
\providecommand{\standardthanksIFMOld}{}
\renewcommand{\standardthanksIFMOld}{Cette recherche a b\'{e}n\'{e}fici\'{e}
  du support financier de la Chaire de recherche du Canada en
  \'{e}conom\'{e}trie, d'une Bourse Guggenheim, de la Bourse Konrad-Adenauer
  (Fondation Alexander von Humboldt, Allemagne),
  de l'Institut de finance math\'{e}matique de Montr\'{e}al
  (IFM2), du Conseil de recherche en sciences humaines du Canada, du
  Conseil de recherche en sciences naturelles et en g\'{e}nie du
  Canada, de la Fondation Alexander von Humboldt (Allemagne), du
  R\'{e}seau canadien de centres d'excellence (projet MITACS), du
  Fonds de recherche sur la soci\'{e}t\'{e} et la culture
  (Qu\'{e}bec), et du Fonds de recherche sur la nature et les
  technologies (Qu\'{e}bec), et d'une Bourse
  Killam (Conseil des Arts du Canada).}

\renewcommand{\Dufouraddress}{William Dow Professor of Economics, McGill University,
  Centre interuniversitaire de recherche en analyse des
  organisations (CIRANO), et Centre interuniversitaire de recherche en
  \'{e}conomie quantitative (CIREQ).  Adresse postale:
  Department of Economics, McGill University, Leacock Building, Room 519,
  855 Sherbrooke Street West, Montr\'{e}al, Qu\'{e}bec H3A 2T7, Canada.
  TEL: (1) 514 398 8879; FAX: (1) 514 398 4938; courriel: jean-marie.dufour@mcgill.ca . Web page:
  http://www.jeanmariedufour.com }
  
  \renewcommand{\DufourAddress}{William Dow Professor of Economics, McGill University,
  Centre interuniversitaire de recherche en analyse des
  organisations (CIRANO), et Centre interuniversitaire de recherche en
  \'{e}conomie quantitative (CIREQ).  Adresse postale:
  Department of Economics, McGill University, Leacock Building, Room 519,
  855 Sherbrooke Street West, Montr\'{e}al, Qu\'{e}bec H3A 2T7, Canada.
  TEL: (1) 514 398 8879; FAX: (1) 514 398 4938; courriel: jean-marie.dufour@mcgill.ca . Web page:
  http://www.jeanmariedufour.com }

\renewcommand{\DufouraddressUM}{Titulaire de la Chaire de recherche du
  Canada en \'{e}conom\'{e}trie (Universit\'{e} de Montr\'{e}al).
  Centre interuniversitaire de recherche en analyse des
  organisations (CIRANO), Centre interuniversitaire de recherche en
  \'{e}conomie quantitative (CIREQ) et D\'{e}partement de sciences
  \'{e}conomiques, Universit\'{e} de Montr\'{e}al. Adresse postale:
  D\'{e}partement de sciences \'{e}conomiques, Universit\'{e} de
  Montr\'{e}al, C.P. 6128 succursale Centre Ville, Montr\'{e}al,
  Qu\'{e}bec, Canada H3C 3J7. TEL: (514) 343 2400; FAX: (514) 343
  5831; courriel: jean.marie.dufour@umontreal.ca. Page Web:
  http://www.fas.umontreal.ca/SCECO/Dufour . }

\renewcommand{\FarhatAddress}{CIRANO et CIREQ.
  Adresse postale: CIREQ, Universit\'{e} de Montr\'{e}al,
  C.P. 6128 succursale Centre-ville, Montr\'{e}al, Qu\'{e}bec, Canada H3C 3J7.
  TEL: 1 514 343 6557; FAX: 1 514 343 5831. \newline  Courriel: abdeljelil.farhat@umontreal.ca.}

\renewcommand{\KhalafAddress}{Titulaire de la Chaire de recherche du Canada
  en Analyse \'econométrique environnementale et financi\`ere (Universit\'e Laval).
  CIREQ, Universit\'{e} de Montr\'{e}al,
  et GREEN, Universit\'{e} Laval. Adresse postale: GREEN, Universit\'{e} Laval, Pavillon J.-A.-De
  S\`{e}ve, St. Foy, Qu\'{e}bec, Canada, G1K 7P4. TEL: (418) 656 2131-2409;
  FAX: (418) 656 7412. Courriel: lynda.khalaf@ecn.ulaval.ca.}

\providecommand{\varnewline}{ \\ }
\renewcommand{\firstversion}[1]{Premi\`ere version: #1 }
\renewcommand{\revised}[1]{\varnewline R\'evisions: #1 }
\renewcommand{\thisversion}[1]{\varnewline Cette version: #1 }
\renewcommand{\compiled}[1]{\varnewline Compil\'e: #1 }
\renewcommand{\dateformat}[3]{Premi\`ere version: #1
 #2 #3 \\ Compil\'e: \today, \now}

\renewcommand{\January}{Janvier }
\renewcommand{\February}{F\'evrier }
\renewcommand{\March}{Mars }
\renewcommand{\April}{Avril }
\renewcommand{\May}{Mai }
\renewcommand{\June}{Juin }
\renewcommand{\July}{Juillet }
\renewcommand{\August}{Ao\^ut }
\renewcommand{\September}{Septembre }
\renewcommand{\October}{Octobre }
\renewcommand{\November}{Novembre }
\renewcommand{\December}{D\'ecembre }

\def\todayMY{\ifcase\month\or
  Janvier\or F\'evrier\or Mars\or Avril\or Mai\or Juin\or
  Juillet\or Ao\^ut\or Septembre\or Octobre\or Novembre\or
  D\'ecembre\fi\ \number\year}

\providecommand{\newpageSlides}{}
\providecommand{\sectitlesize}{}

%% End of  DufourC1F.tex 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> DufourC1SlidesLandscape.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DufourC1SlidesLandscape.tex
%% Latex file 
%% First version: May 18, 2002
%% Revised: 25 July 2016; 25 January 2017
%% Commands for generating slides in landscape form

\usepackage[landscape]{geometry}
\setlength{\totalhormargin}{0.75in}
\setlength{\totalvermargin}{2.0in}
\setlength{\textwidth}{\paperwidth - \totalhormargin}
\setlength{\textheight}{\paperheight - \totalvermargin}
\setlength{\topmargin}{-0.75in} \setlength{\headheight}{0.17in}
\setlength{\headsep}{0.33in} \setlength{\footskip}{0.5in}
\setlength{\oddsidemargin}{-0.75in}
\setlength{\evensidemargin}{0.0in}

\providecommand{\sectitlesize}{\huge}
\renewcommand{\sectitlesize}{\huge}
\providecommand{\newpageSlides}{\newpage}
\renewcommand{\newpageSlides}{\newpage}
\providecommand{\newlineSlides}{\newline}
\renewcommand{\newlineSlides}{\newline}
\providecommand{\slideFontSize}{\LARGE}
\renewcommand{\slideFontSize}{\LARGE}

%% End of DufourC1SlidesLandscape.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
